Relating Misfit to Gain in Weak-to-Strong Generalization Beyond the Squared Loss

The paradigm of weak-to-strong generalization constitutes the training of a strong AI model on data labeled by a weak AI model, with the goal that the strong model nevertheless outperforms its weak supervisor on the target task of interest. For the setting of real-valued regression with the squared loss, recent work quantitatively characterizes the gain in performance of the strong model over the weak model in terms of the misfit between the strong and weak model. We generalize such a characterization to learning tasks whose loss functions correspond to arbitrary Bregman divergences when the strong class is convex. This extends the misfit-based characterization of performance gain in weak-to-strong generalization to classification tasks, as the cross-entropy loss can be expressed in terms of a Bregman divergence. In most practical scenarios, however, the strong model class may not be convex. We therefore weaken this assumption and study weak-to-strong generalization for convex combinations of $k$ strong models in the strong class, in the concrete setting of classification. This allows us to obtain a similar misfit-based characterization of performance gain, upto an additional error term that vanishes as $k$ gets large. Our theoretical findings are supported by thorough experiments on synthetic as well as real-world datasets.

==> arxiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}

\usepackage{yhmath}
\usepackage{amsthm}
\usepackage{amssymb}

\newcommand{\eR}{\overline{\mathbb{R}}}
\newcommand{\eRp}{\overline{\mathbb{R}}^{+}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\inte}{\mathrm{int}}
\newcommand{\intem}[1]{\mathring{\wideparen{#1}}}
\newcommand{\cl}{\overline}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\co}{\mathrm{co}}
\newcommand{\cco}{\overline{\mathrm{co}}}
\newcommand{\xe}{\mathrm{XE}}

\makeatletter
\newcommand{\btriangle}{\mathpalette\btriangle@\relax}
\newcommand{\btriangle@}[2]{%
    \begingroup
    \sbox\z@{$\m@th#1\triangle$}%
    \makebox[\wd\z@]{%
        \raisebox{0.04\height}{%
            \resizebox{1.1\wd\z@}{0.96\ht\z@}{%
                $\m@th#1\blacktriangle$%
            }%
        }%
    }%
    \endgroup
}
\makeatother

\let\ab\allowbreak



==> conclusion.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}


Both the theory in \Cref{sec:main-result} and experiments in \Cref{sec:experiments} raise several questions. Firstly, our empirical results seem significantly tighter than what \Cref{thm:main-result} suggests. Can the proof of \Cref{thm:main-result} be improved to tighten the error term? 
Secondly, can geometric training methods recover $g$ during weak-to-strong learning, given some assumptions on $\mathcal{F}$? For example, if $\mathcal{F}$ is affine, then the weak model could be forced to satisfy an orthogonality constraint so that its Bregman projection onto $\mathcal{F}$ is $g$. Finally, we note that \Cref{thm:main-result} applies to any regularized strong class $\mathcal{F}$ for classification. Our experiments focused on when $\mathcal{F}$ was made up of linear probes \cite{burns2023weaktostronggeneralizationelicitingstrong}, but the theory applies to significantly larger classes of models. %
How tightly does \Cref{thm:main-result} hold in these different settings, and can the ideas from this work be applied there to encourage better alignment?


==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We conduct experiments on synthetic data similar to \citet{charikar2024quantifyinggainweaktostronggeneralization}, and also NLP and Vision datasets considered originally in the work of \citet{burns2023weaktostronggeneralizationelicitingstrong}. %

\subsection{Synthetic Data Experiments}
\label{sec:synthetic-experiments}
We follow the setup in \citet{charikar2024quantifyinggainweaktostronggeneralization} for the synthetic  experiments. We assume that the target $g$ takes the form $f(h^\star(\cdot))$ for some ground-truth representation map $h^\star$ and finetuning function $f \in \gF$. We set $h^\star:\R^8 \to \R^{16}$ to a randomly initialized MLP with 5 hidden layers and ReLU activations, where the hidden size is $16$. We choose $\mathcal{F}$ to be the set of $c$-class logistic regression models on $\R^{16}$. Namely,
\begin{align*}
                       & \gF = \{x \mapsto \sigma(Wx):W \in \R^{(c-1)\times 16}\},                   \\
    \text{where} \quad & \sigma(z^*_1,\dots,z^*_{c-1}):=\mathrm{softmax}([0,z^*_1,\dots,z^*_{c-1}]).
\end{align*}
The marginal $\gP$ of the data is $\gN(0, \nu^2I)$; we set $\nu=100$.

\paragraph{Pretraining.} The class of strong and weak model representations, $\gH_s$ and $\gH_w$, are respectively set to the class of 8-layer and 2-layer MLPs mapping $\R^8 \to \R^{16}$, again with ReLU activations and hidden layer size $16$. To obtain $h_s$ and $h_w$, we first randomly sample $T=10$ maps $f^{(1)},\dots,f^{(T)}$ from $\gF$, and generate data $\{x^{(i)}_j, y^{(i)}_j\}_{j=1}^{N_r}$ for each, where $N_r=2000$. Here, every $x^{(i)}_j \sim \gP$, and $y^{(i)}_j = \sigma(f^{(i)}(h^\star(x^{(i)}_j)))$. Thereafter, the parameters of $h_s$ and $h_w$ are obtained by performing gradient descent to optimize the cross-entropy loss:
\begin{align}
    h_k & = \argmin_{h \in \gH_k} \frac{1}{T N_r}\sum_{i=1}^T\sum_{j=1}^{N_r}\xe(y^{(i)}_j \| \sigma(f^{(i)}(h(x^{(i)}_j)))) \nonumber \\
        & \text{for } k \in \{w,s\}.
\end{align}

\paragraph{Weak Model Finetuning.} Next, we finetune the weak model on $M=100$ fresh finetuning tasks $f^{(1)},\dots,f^{(M)}$ from $\gF$. To do so, we again generate $\{x^{(i)}_j, y^{(i)}_j\}_{j=1}^{N_f}$ for every $i \in [M]$, where $N_f=2000$, each $x^{(i)}_j \sim \gP$ and $y^{(i)}_j = \sigma(f^{(i)}(h^\star(x^{(i)}_j)))$. The weak model representation $h_w$ that was obtained in the pretraining step is held frozen, and the parameters in the final linear layer are obtained via gradient descent to minimize the cross-entropy loss:
\begin{align}
    \label{eqn:synthetic-weak-model-finetuning}
    f^{(i)}_w & = \argmin_{f \in \gF} \frac{1}{N_f}\sum_{j=1}^{N_f}\xe(y^{(i)}_j \|  \sigma(f (h_w(x^{(i)}_j)) ) ).
\end{align}

\paragraph{Weak-to-Strong Supervision.} For each finetuning task above, we obtain data labeled by the weak supervisor as follows. For every $i \in [M]$, we generate  $\{\tilde{x}^{(i)}_j, \tilde{y}^{(i)}_j\}_{j=1}^{N_f}$, where $\tilde{x}^{(i)}_j \sim \gP$ and $\tilde{y}^{(i)}_j = \sigma(f^{(i)}_w(h_w(\tilde{x}^{(i)}_j)))$. This data is fed to the strong model, which goes on to learn:
\begin{align}
    \label{eqn:synthetic-wts-finetuning}
    f^{(i)}_{s} & = \argmin_{\substack{f_1,\dots,f_k \in \gF                            \\ \lambda \in (0,1)^k: \sum_{a}\lambda_a=1}}\frac{1}{N_f}\sum_{j=1}^{N_f}\KL\left(\sum_{a=1}^k \lambda_a  z^{(i,j)}_a \bigg\| \tilde{y}^{(i)}_j\right), \nonumber \\
                & \text{where} \quad z^{(i,j)}_a = \sigma(f_a(h_s(\tilde{x}^{(i)}_j))).
\end{align}
Namely, we optimize over a convex combination of $k$ logistic regression heads. Importantly, observe that the order of arguments in $\KL$ in \Cref{eqn:synthetic-wts-finetuning} above is flipped from that in \Cref{eqn:synthetic-weak-model-finetuning}, in keeping with the recipe given by \Cref{thm:main-result}. We set $k=100$.

\paragraph{Evaluation.} To evaluate that the inequality given by \Cref{thm:main-result} holds, for each task $i \in [M]$, we estimate the three expectations in \Cref{eqn:misfit-inequality-evaluation} from a new sample of size $N_f$. Our result says that upto an error term of $O(\sqrt{c/k})$, %
\begin{align}
    \label{eqn:synthetic-pythagorean-inequality}
     & \E\left[\xe(g(X) \| f_w ( h_w(X)))\right] - \E \left[\xe(g(X) \| f_s ( h_s(X)))\right] \nonumber \\
     & \qquad\ge \E \left[\KL(f_s ( h_s(X)) \| f_w (h_w(X)))\right].
\end{align}
In \Cref{fig:synthetic-experiments}, we plot the LHS on the y-axis and the RHS on the x-axis, for the experiment above performed with $c=2,10,50,100$. We can observe that \Cref{eqn:synthetic-pythagorean-inequality} is exhibited more or less with equality, for both the binary $(c=2)$ as well as multiclass cases $(c>2)$. We do note that the plot gets noisier as $c$ grows to $100$. These plots show the same trend as for the squared loss in \citet{charikar2024quantifyinggainweaktostronggeneralization}.
\begin{figure*}[t]
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/2-5-8-binary-k-100.pdf}
        \caption{$c=2$}
        \label{fig:2-5-8-binary}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/2-5-8-multiclass-9-k-100.pdf}
        \caption{$c=10$}
        \label{fig:2-5-8-multiclass-10}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/2-5-8-multiclass-49-k-100.pdf}
        \caption{$c=50$}
        \label{fig:2-5-8-multiclass-50}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/2-5-8-multiclass-99-k-100.pdf}
        \caption{$c=100$}
        \label{fig:2-5-8-multiclass-100}
    \end{subfigure}
    \caption{Synthetic data experiments. The Gain and Misfit closely track each other. For $c=100$, we see that the correlation between misfit and gain weakens, suggested also by the $O(\sqrt{c / k})$ error term from \Cref{thm:multi-main-result}.}
    \label{fig:synthetic-experiments}
\end{figure*}

\subsection{NLP Tasks}
\label{sec:nlp-experiments}

\begin{figure*}[t]
    \begin{subfigure}{.24\textwidth}
        \centering
        \caption{CosmosQA}
        \includegraphics[width=1\linewidth]{arxiv/img/cosmos_qa_gpt2.pdf}
        \label{fig:cosmos-qa-gpt2}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \caption{Amazon Polarity}
        \includegraphics[width=1\linewidth]{arxiv/img/amazon_polarity_gpt2.pdf}
        \label{fig:amazon-polarity-gpt2}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \caption{BoolQ}
        \includegraphics[width=1\linewidth]{arxiv/img/boolq_gpt2.pdf}
        \label{fig:boolq-gpt2}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \caption{SciQ}
        \includegraphics[width=1\linewidth]{arxiv/img/sciq_gpt2.pdf}
        \label{fig:sciq-gpt2}
    \end{subfigure}
    \caption{Weak model (\texttt{gpt2}) is trained once on true labels and thereafter fixed. Each strong model is trained on the weak labels (on a held-out set separate from that which weak model was trained on) for 10 random initializations of the $k$-convex combination of logistic regression heads; we plot the average test loss/misfit across these 10 runs, along with the standard deviations as the error bars.}
    \label{fig:gpt2-weak-model}
\end{figure*}

Next, we consider four real-world NLP classification datasets\footnote{These are four of the five datasets considered in the codebase provided by OpenAI \citep{ecoffet2023} for their weak-to-strong generalization paper. We chose to not include the fifth (Anthropic/HH-RLHF \citep{bai2022training, ganguli2022red}) since the results of \citet{burns2023weaktostronggeneralizationelicitingstrong} on this dataset are extremely noisy (see the plot in \citet{ecoffet2023}), e.g., no model seems to be doing better than random guessing.}: BoolQ \citep{clark2019boolq}, SciQ \citep{welbl2017crowdsourcing}, CosmosQA \citep{huang2019cosmos} and Amazon Polarity \citep{mcauley2013hidden}. %
We work with models in the \texttt{gpt2} family \citep{gpt2}, where the weak model is fixed to be \texttt{gpt2}, and the strong model is chosen from \texttt{gpt2-medium}, \texttt{gpt2-large} and \texttt{gpt2-xl}. For each dataset, we first finetune the linear probe of the weak model (by minimizing cross-entropy) on 50\% of the training data with ground-truth labels. We then compute weak labels given by the trained model on the remaining 50\% of the training data. We then optimize a convex combination of $k=100$ logistic regression heads on top of the strong model to minimize the reverse objective as in \Cref{eqn:synthetic-wts-finetuning}. We add an $\ell_2$ regularization penalty (with coefficient 0.1) on the linear weights in the objective to help with regularization, and to better align with the requirements of \Cref{thm:main-result}. Finally, we estimate each of the terms in \Cref{eqn:synthetic-pythagorean-inequality} from the test data. The obtained results are shown in \Cref{fig:gpt2-weak-model}.

Firstly, we see weak-to-strong generalization (in terms of the loss) for all the datasets: the test loss of the strong model is always smaller than the test loss of its weak supervisor. Next, we see a clear trend on all four datasets: as we range the strong model from \texttt{gpt2-medium} to \texttt{gpt2-large} to \texttt{gpt2-xl}, the misfit onto the weak model increases, and concurrently, the loss on the test data decreases. In fact, for CosmosQA, Amazon Polarity and SciQ, in addition to the test loss decreasing, we observe that the test \textit{accuracy} is non-decreasing too (note again that our result does not claim anything about accuracy per se).

We remark that our accuracies are inferior to those reported in the experiments by \citet{burns2023weaktostronggeneralizationelicitingstrong} on these datasets. One reason for this is that we only ever tune the logistic regression heads of models (in both weak model training, as well as weak-to-strong training), whereas \citet{burns2023weaktostronggeneralizationelicitingstrong} allow full finetuning that includes the representation layer parameters. Additionally, our objective in the weak-to-strong training procedure is not the standard cross-entropy (which would have formed a convex objective w.r.t. the logistic regression parameters), but the reverse KL divergence objective given in \Cref{eqn:synthetic-wts-finetuning}. The latter is a non-convex objective, which can cause difficulty in minimizing the loss.

\subsection{Vision Tasks}
\label{sec:vision-experiments}

\begin{figure*}[t]
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/cifar-10_alexnet.pdf}
        \caption{CIFAR-10}
        \label{fig:cifar-10_alexnet}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/imagenet_alexnet.pdf}
        \caption{ImageNet}
        \label{fig:imagenet_alexnet}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/consolidated-k.pdf}
        \caption{Varying $k$}
        \label{fig:varying-k}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{arxiv/img/consolidated-realizable.pdf}
        \caption{Consolidated misfit/gain plot across all datasets.}
        \label{fig:consolidated-realizable}
    \end{subfigure}
    \caption{(a), (b) Weak model (AlexNet) is trained once on true labels and thereafter fixed; we report numbers averaged over 10 runs of weak-to-strong training. (c) We observe that the difference between misfit and gain decreases as $k$ increases, and also that the decrease slows down with increasing $k$. (d) The test loss of the weak and strong model is measured not with respect to the ground truth test data, but instead with respect to the predictions of the best strong model on the test data. This is done to ensure realizability.}
    \label{fig:vision-consolidated}
\end{figure*}

We next perform experiments on image classification datasets. Following \citet{burns2023weaktostronggeneralizationelicitingstrong}, we fix the weak supervisor to be AlexNet \citep{krizhevsky2012imagenet}. For the strong model, we consider ResNet-50 \citep{he2016deep} and ViT-B/8 \citep{dosovitskiy2020image} based on DINO representations \citep{caron2021emerging}. Having fixed these representations, we finetune a convex combination of $k=100$ logistic heads on top of the strong model on the weakly labeled data. We consider two datasets: CIFAR-10 \citep{krizhevsky2009learning} and ImageNet \citep{ILSVRC15}, and obtain the same plots as we did for the NLP datasets in Figures \ref{fig:cifar-10_alexnet}, \ref{fig:imagenet_alexnet}. Again, we clearly observe that as the misfit of the strong model onto the weak labels increases, both, the test loss decreases as well as the test accuracy increases! Interestingly, we observe that our weak-to-strong accuracy on ImageNet for ViT-B/8 is \textit{better than} the corresponding weak-to-strong accuracy reported for the same experiment in Table 3, \citet{burns2023weaktostronggeneralizationelicitingstrong} (namely 64.2\% respectively). We note that the only difference in our setup is the weak-to-strong training of the linear probe: while \citet{burns2023weaktostronggeneralizationelicitingstrong} adopt standard cross-entropy minimization on a single logistic head, we employ the reverse KL minimization on a convex combination of $k$ heads, as suggested by our theory. Empirically benchmarking these two slightly different weak-to-strong training methods constitutes an interesting future direction.

\subsection{Varying $k$}
Recall that with a convex combination of $k$ logistic heads, the upper bound on the difference between misfit and gain in \Cref{thm:multi-main-result} scales as $O(\sqrt{c/k})$; in particular, as $k$ increases, the upper bound becomes smaller. As our next experiment, for each dataset, we fix the strong model to be the largest one (\texttt{gpt2-xl} for NLP, and ViT-B/8 for Vision), and vary $k$ in $\{1,10,50,100\}$. For each dataset, we plot the difference between misfit and gain against $k$; the plots are shown in \Cref{fig:varying-k-all-plots} in \Cref{sec:plots-varying-k}. We observe that for all datasets but ImageNet, the difference between misfit and gain consistently decreases as $k$ increases; furthermore, beyond a point, increasing $k$ does not decrease the discrepancy by much. This can also be seen in \Cref{fig:varying-k}, which collates the plots for all datasets (except ImageNet) in a single figure.\footnote{We chose to not include ImageNet in this plot as the plot for ImageNet was significantly off scale, and was skewing the y-axis.} We suspect that the trend does not show up for ImageNet because  $c=1000$, and hence $c$ dominates in the error term for the values of $k$ that we consider.


\subsection{Enforcing the Realizability Assumption}
Finally, while the plots in \Cref{fig:gpt2-weak-model} and \Cref{fig:cifar-10_alexnet}, \ref{fig:imagenet_alexnet} do illustrate that the gain in performance is directly proportional to the misfit as expected, our theory would also additionally suggest that the gain should \textit{quantitatively} be at least the misfit (up to an error term decreasing in $k$). This does not quite hold in the plots---we can observe that the misfit is consistently larger than the difference between the weak model and strong model loss.
One significant reason for this is that our result assumes realizability; namely, the target task should be \textit{exactly} representable by the strong model. %
We verified that this does not actually hold in our experiments---even if we train the strong models on data with ground-truth labels, we see a non-trivial test loss at the end of training. To isolate this cause of discrepancy,
we can consider evaluating the test losses of the weak and strong models (two terms on the LHS of \eqref{eqn:synthetic-pythagorean-inequality}) with respect to the best possible strong model (that is trained on true labels) instead of the ground-truth target function. This simply ensures that the realizability assumption holds. If we evaluate the quantities thus, consolidate the numbers across all the different NLP and vision datasets, and plot them with axes as in \Cref{fig:synthetic-experiments}, we obtain \Cref{fig:consolidated-realizable}. Note how this plot is more aligned to the plots in \Cref{fig:synthetic-experiments}, with the misfit more faithfully capturing the quantitative gain in performance. %


==> introduction.tex <==
\section{Introduction} \label{sec:introduction}


The premise in weak-to-strong generalization \citep{burns2023weaktostronggeneralizationelicitingstrong} is that increasingly strong AI models will learn to outperform their weak supervisors, even when they are trained on data labeled by these weak supervisors. By virtue of being larger and more complex models that have presumably also seen more data in their pretraining lifecycle, the hope is that strong models will invariably know to push past the performance ceiling of their weak supervisors. This phenomenon is central towards the eventual goal of superalignment \citep{superalignment}, where we expect AI models to exhibit superhuman skills aligned with human principles from human supervision. Perhaps encouragingly, recent studies \citep{burns2023weaktostronggeneralizationelicitingstrong, guo2024vision, ji2024aligner, sun2024easy, yang2024weak, zhang2024transcendence, liu2024co} have affirmed that such a phenomenon can in fact be elicited. Given the extent to which emergent AI would appear to influence our future going forward, it becomes imperative to theoretically understand when and how weak-to-strong generalization may provably be exhibited.


Towards this, a recent work by \citet{charikar2024quantifyinggainweaktostronggeneralization} provides a mathematical characterization of weak-to-strong generalization for the specific task of real-valued regression. The setting in this work considers finetuning the final linear layer of a strong model (keeping other parameters fixed) to minimize the squared loss on labels given by a weak model. Using a geometric argument involving projections onto a convex set, \citet{charikar2024quantifyinggainweaktostronggeneralization} show that a strong model trained in this manner provably attains smaller loss than the weak model on the target task. Moreover, the quantitative reduction in the loss (equivalently, the performance ``gain'') is at least as much as the loss of the strong model on the weakly labeled data, or rather the ``misfit''\footnote{This notion of misfit is also referred to as ``student-supervisor disagreement'' in \citet{burns2023weaktostronggeneralizationelicitingstrong}.} between the strong and weak model. Notably, \citet{charikar2024quantifyinggainweaktostronggeneralization} only obtain results for regression, leaving open whether such misfit-based characterization for weak-to-strong generalization can also be formally shown for other tasks, including the standard task of classification, which was one of the primary subjects of study in \citet{burns2023weaktostronggeneralizationelicitingstrong}.


In this work, inspired by the theory of information geometry \citep{amari2016information, Ay2017}, we significantly extend the misfit-based characterization of the performance gain in weak-to-strong generalization beyond regression tasks. Our main observation is that the Pythagorean inequality for the squared loss that is used to establish the result in \citet{charikar2024quantifyinggainweaktostronggeneralization} holds more generally for \textit{Bregman divergences} \citep{bregman1967relaxation}. Thus, whenever the loss function in the learning task is a Bregman divergence of some kind, a corresponding misfit-based weak-to-strong generalization inequality can be established. For example, since the squared $\ell_2$ distance is a Bregman divergence, the result of \citet{charikar2024quantifyinggainweaktostronggeneralization} constitutes a special case of this theory. More importantly, the standard loss function that is used in classification tasks, namely cross-entropy, can also be written down as a Bregman divergence (namely the Kullback-Leibler (KL) divergence \citep{kullback1951information}) plus an additive entropy term. This lets us derive a recipe for provable weak-to-strong generalization in the setting of classification (in the sense that the cross-entropy loss provably reduces), along with a misfit-based characterization of the gain similar to \citet{charikar2024quantifyinggainweaktostronggeneralization}.


Our recipe for guaranteeing provable weak-to-strong generalization is however somewhat non-standard, and possibly counterintuitive: optimize a convex combination of $k$ logistic regression layers on top of the strong model representation to minimize the expected KL divergence between the strong model's output and the weak labels. Notably, the strong model's output is in the \textit{first} argument in the KL divergence---contrast this to standard supervised classification with the cross-entropy loss, where instead, the supervisor's labels are in the first argument of the cross-entropy (and consequently, the KL divergence). In this sense, our recipe is asking to minimize the discrepancy between the supervisor (weak model) and student (strong model), but in the \textit{opposite} direction. Nevertheless, for sufficiently large values of $k$, doing so provably results in smaller cross-entropy between the ground-truth data and the strong model (which is what we actually care about) than the cross-entropy between the ground-truth data and the weak model. Furthermore, the reduction in the loss is at least the KL divergence between the strong model and the weak model at the conclusion of weak-to-strong training! Thus, performance gain can yet again be measured in terms of the misfit between the strong and weak models, albeit with the notion of misfit here being the KL divergence.

We validate our theory across synthetic as well as real-world NLP and Vision datasets, and find that when the strong model is trained according to the stated recipe even with modest values of $k$ (e.g., 100), its performance gain is faithfully characterized by its KL misfit with the weak model. Additionally, this behavior becomes more apparent as $k$ increases, further validating our theory.



==> main-result.tex <==
\section{Main Results} \label{sec:main-result}

We are now in a position to state our main results on weak-to-strong generalization using Bregman divergence theory. %

The first result is a direct application of ~\Cref{thm:bg_pyth_main}.

\begin{theorem}[Bregman Misfit-Gain Inequality] \label{thm:main-result-conv-bg}
    Let $\psi: \sR^n \to \eRp$ be a proper convex function s.t. $U_\psi \neq \emptyset$. Let $h_s: \mathcal{X} \to \sR^{d_s}$ and $h_w: \mathcal{X} \to \sR^{d_w}$ be the strong and weak learner representations respectively. Let $f_w: \sR^{d_w} \to U_\psi$ be the weak model finetune layer, and $g: \mathcal{X} \to U_\psi$ be the target function. Let $\mathcal{F}$ be a class of functions mapping $\sR^{d_s} \to U_\psi$. If the following hold:
    \begin{enumerate}
        \item (Realizability) $\exists f_* \in \mathcal{F}$ s.t. $g = f_* \circ h_s$,
        \item (Convexity) $\mathcal{F}$ is a convex set of functions,
        \item (Sequential Consistency) For $y \in U_\psi$ fixed, if $D_{\psi}(x_n, y) \to 0$, then $x_n \to y$,
    \end{enumerate}
    then for any $\epsilon > 0$, there exists $\delta > 0$ such that for all $f_s \in \mathcal{F}$ that satisfy
    \begin{align*}
        \E \big[ D_{\psi} & \left( f_s(h_s(X)) , f_w( h_w(X)) \right) \big]                                                                        \\
                                    & \leq \inf_{f \in \mathcal{F}} \E \left[ D_{\psi}\left(f( h_s(X) ) , f_w ( h_w(X) ) \right) \right] + \delta,
    \end{align*}
    we have
    \begin{align} \label{eq:misfit-ineq-bg}
        \E \big[D_{\psi} & \left(g(X) , f_s(h_s(X)) \right) \big] \nonumber                                     \\
        \leq                    & \; \E \left[D_{\psi}\left(g(X) , f_w(h_w(X))\right)\right] \nonumber            \\
                                & - \E \left[D_{\psi}\left(f_s(h_s(X)) , f_w(h_w(X))\right)\right] + \epsilon.
    \end{align}

\end{theorem}
\begin{proof}[Proof Sketch]
    Because $\mathcal{F}$ is convex, we get that $\mathcal{F} \circ h_s$ is also convex. Since $g \in \overline{\mathcal{F} \circ h_s}$, by \Cref{thm:bg_pyth_main}, we have that $g_{\text{proj}} := P_{\overline{\mathcal{F} \circ h_s}}(f_w \circ h_w)$ uniquely exists and satisfies the Bregman Pythagorean inequality. Now, by continuity of both $\E[D_{\psi}(\cdot  , f_w(h_w(X)))]$ and $\E[D_{\psi}(g(X) , \cdot)]$ there exists an $\epsilon_1 > 0$ s.t. if $\E \left[ \|f(h_s(X)) - g_{\text{proj}}(X)\|_2^2 \right] < \epsilon_1$, then $f$ almost satisfies the Pythagorean inequality with error $\epsilon$. Choosing $\delta$ sufficiently small, we can apply the Pythagorean inequality to bound $\E [D_{\psi} (f(h_s(X))  , g_{\text{proj}}(X))]$. Sequential consistency will then make $\E \left[ \| f(h_s(X)) - g_{\text{proj}}(X)\|_2^2 \right] < \epsilon_1$.
\end{proof}

Sequential consistency is a common assumption in the literature when defining Bregman divergences \cite{Reem_2018, Bauschke2003, Butnariu2003}, and is satisfied with very weak assumptions on $\psi$. ~\cref{thm:main-result-conv-bg} generalizes Theorem~1 in \citet{charikar2024quantifyinggainweaktostronggeneralization}, since $\ell_2$ is a Bregman divergence (and clearly sequentially consistent).

As a corollary to Theorem~\ref{thm:main-result-conv-bg}, we also obtain the misfit-gain inequality for cross-entropy.

\begin{corollary}[Cross-Entropy Misfit-Gain Inequality]
    \label{thm:main-result-conv}
    Let $h_s: \mathcal{X} \to \sR^{d_s}$ and $h_w: \mathcal{X} \to \sR^{d_w}$ be the strong and weak model representations respectively. Let $g: \mathcal{X} \to (0,1)$ be the target function. Let $\mathcal{F}$ be a class of functions mapping $\mathbb{R}^{d_s} \to (0,1)$. Let $f_w: \mathbb{R}^{d_w} \to (0,1)$ be the classifier for the weak model. If the following hold:
    \begin{enumerate}
        \item (Realizability) $\exists f_* \in \mathcal{F}$ so that $g = f_* \circ h_s$,
        \item (Convexity) $\mathcal{F}$ is a convex set of functions,
    \end{enumerate}
    then for any $\epsilon > 0$, there exists $\delta > 0$ such that for all $f_s \in \mathcal{F}$ that satisfy
    \begin{align*}
        \E \big[ &\KL(  f_s (h_s(X)) \| f_w ( h_w(X) )) \big]                                                                           \\
                              & \leq \; \inf_{f \in \mathcal{F}} \E\left[ \KL\left(f ( h_s(X) ) \| f_w ( h_w(X) )\right) \right] + \delta,
    \end{align*}
    we have
    \begin{align} \label{eq:misfit-ineq}
        \E\big[\xe & (g(X) \| f_s ( h_s(X) )) \big] \leq \E \left[\xe\left(g(X) \| f_w ( h_w(X) )\right)\right] \nonumber               \\
                           & - \E \left[\KL\left(f_s ( h_s(X) ) \| f_w ( h_w(X) )\right)\right] + \epsilon.
    \end{align}
\end{corollary}
\begin{proof}[Proof Sketch]
    We can first rewrite \Cref{eq:misfit-ineq} in terms of $\KL$ instead of $\xe$ by subtracting $H(g(X))$ from both sides. Since $\KL$ is sequentially consistent by Pinsker's inequality, we can apply Theorem~\ref{thm:main-result-conv-bg}.
\end{proof}

We note that if $$f_s = \argmin_{f \in \mathcal{F}} \E\left[ \KL(f  (h_s(X)) \| f_w ( h_w(X))) \right],$$ then \Cref{eq:misfit-ineq} directly holds with no $\epsilon$ term. Such an $f_s$ uniquely exists if $\mathcal{F} \circ h_s$ is closed. We refer to $\E \left[\KL(f_s(h_s(X)) \| f_w(h_w(X)))\right]$ as the ``misfit'' term and $\E\left[\xe(g(X) \| f_w (h_w(X)))\right] -  \E\left[\xe(g(X) \| f_s( h_s(X)))\right]$ as the ``gain'' term.


In practice, $\mathcal{F}$ is usually not convex. For example, when learning a linear probe \cite{burns2023weaktostronggeneralizationelicitingstrong} on top of $h_s$ together with the sigmoid, $\mathcal{F}^*$ is convex, but $\mathcal{F}$ itself is not. Nevertheless, our main observation in this case is that Theorem~\ref{thm:main-result-conv} still applies to $\co \mathcal{F}$! By Caratheodory's theorem, $\co \mathcal{F} = \co^{|\mathcal{X}| + 1} \mathcal{F}$, and hence we can simply consider convex combinations of $|\mathcal{X}| + 1$ functions in $\mathcal{F}$ to represent $\co \mathcal{F}$. However, as $|\mathcal{X}| \to \infty$, this representation is not computationally tractable. We therefore suggest remedying this by attempting to project the weak model onto $\co^k \mathcal{F} \circ h_s$, and show that the error in the misfit-gain inequality can still be bounded by a decreasing function in $k$ that is independent of $|\mathcal{X}|$. Concretely, we show that:

\begin{theorem} \label{thm:main-result}
    Let $h_s, h_w, f_w, g$ be as in Theorem~\ref{thm:main-result-conv}. Let $\mathcal{F}$ be a class of functions mapping $\R^{d_s} \to (0,1)$. If the following hold
    \begin{enumerate}
        \item (Realizability) $\exists f_* \in \mathcal{F}$ so that $g = f_* \circ h_s$,
        \item (Regularization) $\mathcal{F}$ satisfies $$\max\left( \E \left[\sup_{f \in \mathcal{F}} 1/f(X) \right], \E \left[ \sup_{f \in \mathcal{F}} 1/\overline{f(X)}) \right] \right) < \infty,$$
    \end{enumerate}
    then for any $k \in \sN$, there exists $\delta > 0$ such that for all $f_s \in \co^k \mathcal{F}$ that satisfy
    \begin{align*}
        \E \big[ \KL(&f_s  (h_s(X)) \| f_w (h_w(X))) \big]                                                             \\
        \leq             &\;  \inf_{f \in \co^k \mathcal{F}} \E\left[ \KL(f ( h_s(X)) \| f_w  (h_w(X))) \right] + \delta,
    \end{align*}
    we have
    \begin{align}
        \label{eqn:misfit-inequality-evaluation}
        \E&\big[  \xe(g(X) \| f_s ( h_s(X)))\big] \leq \E \left[\xe(g(X) \| f_w ( h_w(X)))\right] \nonumber \\
                & - \E \left[\KL(f_s ( h_s(X)) \| f_w (h_w(X)))\right] + O(1/\sqrt{k}).        
    \end{align}
\end{theorem}

The proof of ~\Cref{thm:main-result}, inspired from the work of \citet{ZEEVI199799}, is more involved, and is a careful application of the probabilistic method; we defer it to the Appendix as Theorem~\ref{thm:multi-main-result} where we prove it in the multi-class setting; in particular, with $c$ classes, the error term becomes $O(\sqrt{c / k})$. %

We note that both ~\Cref{thm:main-result-conv,,thm:main-result} make no assumption on the weak model, and only the realizability assumption on the target. Theorem~\ref{thm:main-result} makes only a mild assumption on $\mathcal{F}$ that can be enforced by regularizing the models in $\mathcal{F}$ (e.g., via an $\ell_2$ penalty). We emphasize however that the inequality does not guarantee \textit{significant} weak-to-strong generalization for any weak model. If $f_w \in \mathcal{F}$, %
then the $f_s$ obtained by either theorems will be $f_w$ itself, and the misfit term becomes $0$. However, ~\Cref{thm:main-result-conv,,thm:main-result} allow us to \textit{quantify} how much weak-to-strong generalization we should expect to see. All expectations involved can be estimated on a hold-out dataset, yielding a bound on the gain in terms of empirical misfit, modulo estimation error. This quantification is in the \textit{loss} of the learned strong model relative to the (realizable) ground truth data. Since a reasonable loss function is correlated with other error metrics like accuracy, we should expect to empirically see improvements in accuracy with increases in loss misfit. However, a relationship between accuracy and loss misfit is \textit{not} theoretically guaranteed.

\Cref{thm:main-result} provides a concrete recipe for weak-to-strong generalization that allows for a quantitative handle on the performance gap between the weak and strong model. In this recipe, we finetune a convex combination of $k$ functions from $\mathcal{F}$ on top of the strong model representation. The objective of this finetuning is the empirical mean of the KL divergence between the strong and weak model output. Importantly, the strong model's output is in the \textit{first} argument of the KL divergence. This is in contradistinction to the standard weak supervision objective, wherein the weak supervisor's output is in the first argument. However, this distinction provably leads to a performance gain, provided $k$ is not too small, and the empirical estimates are accurate. In the next section, we empirically validate this recipe.









==> preliminaries.tex <==
\section{Preliminaries} \label{sec:preliminaries}

We begin by formally describing the weak-to-strong generalization setup, adopting notation from \citet{charikar2024quantifyinggainweaktostronggeneralization}).



\subsection{Weak-to-strong Generalization}

The setup constitutes a ``strong model'' and a ``weak model'', where the strong model is typically a larger, and representationally more powerful AI model than the weak model. The weak model plays the role of teacher and the strong model plays the role of student, in that the strong model is trying to learn a target function from (potentially inaccurate and noisy) evaluations made by the weak model on data. Abstractly, we think of the strong and weak models via their representation maps $h_s:\mathcal{X}\to \mathbb{R}^{d_s}$ and $h_w:\mathcal{X}\to \mathbb{R}^{d_w}$ respectively on the data domain $\mathcal{X}$. For example, $h_s$ could be a deep transformer architecture, and $h_w$ a shallow architecture. Suppose $g: \mathcal{X} \to \mathcal{Y}$ is some target function. The only signal that the strong model gets about $g$ is through evaluations of the weak model on data. Namely, it sees a dataset labeled by $f_w(h_w(\cdot))$, where $f_w:\mathbb{R}^{d_w}\to \mathcal{Y}$ is a finetuning map that the weak model has obtained, possibly after seeing a different batch of data labeled by $g$ itself. Importantly, the labels that the weak model feeds to the strong model is from a separately held-out dataset, so that the weak model does not have access to the true labels for it. The objective of the strong model then is to obtain a finetuning function $f_s$ for itself that it can compose onto its representation $h_s$, such that $f_s(h_s(\cdot))$ estimates $g$ \textit{better} than $f_w(h_w(\cdot))$.

For the theory in the main body of the paper, we make two assumptions to avoid measure-theoretic and functional-analytic complications and to simplify the exposition: (1) we assume all distributions have finite support, and (2) we restrict our attention to binary classification rather than $c$-ary classification for $c > 2$.
The main results can be generalized when $(1)$ is relaxed; however, more involved technical machinery is required (see \Cref{sec:beyond-finite}). Only minor modifications are needed when $(2)$ is relaxed (see \Cref{sec:multiple_classes}). We now set up some notation.

\subsection{Notation}
For $n \in \sN$, we denote $[n] := \set{1, \dots, n}$. $\eRp := \sR \cup \set{\infty}$. %
For a class of functions $\mathcal{F}$ and a function $h$, we write $\mathcal{F} \circ h$ for the set $\set{f \circ h}_{f \in \mathcal{F}}$. If $f$ is a function, we write $f \equiv c$ if $f$ is constantly $c$. For $p \in [0,1]$, denote $\overline{p} := 1-p$. All logarithms are taken with base $e$. $H: [0,1] \to [0, \log 2]$ is the binary Shannon entropy $H(p) := -p \log p - \overline{p} \log \overline{p}$. $\KL: [0,1]^2\to \eRp$ is the binary KL-divergence $\KL(p \| q) := p \log \frac{p}{q} + \overline{p} \log \frac{\overline{p}}{\overline{q}}$, and $\xe: [0,1]^2 \to \eRp$ is the binary cross-entropy $\xe(p \| q) := -p \log q - \overline{p} \log \overline{q}$. Note that $\xe(p \| q) = \KL(p \| q) + H(p)$. $\sigma: \sR \to (0,1)$ denotes the sigmoid function $\sigma(x) := \frac{e^x}{1 + e^x}$, and $\sigma^{-1}$ is its inverse, the logit function.

For a subset $S \subset \sR^n$, $\inte S$ denotes its interior, and $\overline{S}$ its closure. $\co S$ is its convex hull which is the intersection of all convex sets containing $S$, and $\cco S$ is its closed convex hull which is the intersection of all \textit{closed} convex sets containing $S$. Note $\cco S = \overline{\co S}$. The convex hull of a set can be expressed as the set of all $k$-convex combinations of points in $S$, with $k$ ranging through $\sN$. We use $\co^k S$ to denote all convex combinations of any $k$ elements of $S$.

We use capital letters for random variables. These are instantiated by specifying a distribution (e.g., $X \sim P_X$ signifies random variable $X$ is drawn with probability distribution $P_X$). As mentioned above, all distributions are assumed to have finite support. For a function $f$ of a random variable, $\E_X[f(X)]$ denotes the expectation of $f(X)$ over $P_X$. When no subscript is attached to $\E$, the expectation is taken with respect to all random variables in scope. The probability distribution of a random variable $X$ is written as $P_X$. For a pair of random variables $X,Y$ jointly distributed, the conditional distribution of $Y$ given $X$ is notated as $P_{Y | X}$.



\subsection{Convexity}

We will take for granted many basic results about convex functions; \citet{ekeland1999convex} is a good reference for these. For a convex function $\psi: \sR^n \to \eRp$, we write $\dom \psi$ for  $\set{x \in \R^n : \psi(x) < \infty}$. A convex function is \textit{proper} if $\dom \psi \neq \emptyset$. All convex functions in this paper will be assumed to be proper. We denote $U_\psi := \inte \dom \psi$. Over $\R^n$, all convex functions with nonempty domain are continuous over $U_\psi$. When $\psi: \sR^n \to \eRp$ is strictly convex and $C^1(U_\psi)$, $\nabla \psi$ is a homeomorphism onto its image, and plays an important role in the theory of convex duality. When such a $\psi$ is specified, we denote $x^* := \nabla \psi(x)$ for $x \in U_\psi$. Likewise, for $S \subset U_\psi$, $S^* := \nabla \psi(S)$. The Legendre dual of such a $\psi$ is $\psi^* : \R^n \to \eRp$, where $\psi^*(x^*) := \langle x, x^* \rangle - \psi(x)$ for $x \in U_\psi$, and $\infty$ otherwise. %
It is also a strictly convex function that is $C^1$ on $U_{\psi^*} = (U_\psi)^*$. Furthermore, $\psi^{**} = \psi$, and $\nabla \psi^* = (\nabla \psi)^{-1}$. As such, When $\psi$ and $\psi^*$ are distinguished, we call $U_{\psi}$ the primal space and $U_{\psi^*}$ the dual space. We refer to $\nabla \psi$ as the dual map, and $x^*$ the dual of $x \in U_{\psi}$.





\subsection{Bregman Divergences}

Our primary means of generalizing beyond the squared loss analyzed in \citet{charikar2024quantifyinggainweaktostronggeneralization} to cross-entropy and other loss functions is via Bregman divergences \cite{bregman1967relaxation}.
\begin{definition}[Bregman Divergence]
    Let $\psi: \sR^n \to \eRp$ be a strictly convex and $C^1(U_\psi)$. Then the $\psi$-Bregman divergence, $D_{\psi}: \sR^n \times U_{\psi} \to \eRp$ is defined
    \begin{align*}
        D_{\psi}(x, y) & := \psi(x) - \psi(y) - \langle x - y, y^* \rangle \\
                       & = \psi(x) + \psi^*(y^*) - \langle x, y^* \rangle.
    \end{align*}
\end{definition}

Here, $\psi$ is the \textit{generator} of $D_{\psi}$. Intuitively, $D_\psi$ measures how much the linear approximation of $\psi$ at $y$ underestimates $\psi(x)$. It is always nonnegative, and is $0$ if and only if $x = y$. The alternative expression for $D_{\psi}$ also reveals an important property: $D_{\psi}(x,y) = D_{\psi^*}(y^*, x^*)$.
Furthermore, $D_{\psi}$ is strictly convex and differentiable in its first argument. This makes it a desirable loss function in optimization algorithms \cite{Collins2002, orabona2023modernintroductiononlinelearning}.

Many commonly used loss functions arise as Bregman divergences (see ~\Cref{table:bg-ex} in \Cref{sec:bregman-divergences-table}).
While Bregman divergences are convex in their first argument, they are \textit{not necessarily} convex in their second argument. The logistic cost (\Cref{table:bg-ex}) is an example of this.

\subsubsection{Cross-Entropy and KL-Divergence}
In binary classification tasks, we work with data $X,Y \sim P_{X,Y}$, where input data $X \in \sR^d$ and labels $Y \in \set{0,1}$. Let $g: \R^d \to [0,1]$ be the conditional probability function $g(x) := P_{Y|X}(1 | x)$. Given some hypothesis class $\mathcal{F}$ of functions $\sR^d \to (0,1)$, we wish to find an $f \in \mathcal{F}$ that minimizes $\E[ \xe(g(X) \| f(X))]$. Since $g$ is fixed for a given classification task, we see that $\E[\xe(g(X) \| f(X))]$ differs from $\E[\KL(g(X) \| f(X))]$ by the task-dependent constant $\E[H(g(X))]$. Thus, for classification tasks, \textit{applying Bregman divergence theory will produce corresponding results about cross-entropy, modulo a constant}. This is the primary justification for using Bregman divergences to understand weak-to-strong learning for classification.






\subsubsection{Geometry of Bregman Divergences}

We would like to use Bregman divergences analogously to distances like the $\ell_2$ distance. However, Bregman divergences are not always symmetric. The KL-divergence is a classic example of a non-symmetric Bregman divergence. Thus, they are not valid distances. However, they do possess many geometric properties. We use two properties below to generalize the main result from~\citet{charikar2024quantifyinggainweaktostronggeneralization}. Below, $\psi$ refers to a strictly convex, $C^1(U_{\psi})$ function.

\begin{fact}[Generalized Law of Cosines \cite{chen-convergence}] \label{thm:cosines}
    Let $x,y,z \in U_\psi$. Then
    $$D_\psi(x, z) = D_\psi(x, y) + D_\psi(y, z) - \langle x - y, z^* - y^* \rangle.$$
\end{fact}

To generalize the Pythagorean inequality for inner product spaces, we need the following notion
\begin{definition}
    Let $\mathcal{W} \subset U_{\psi}$. For $x \in U_{\psi}$, define the forward Bregman projection to be $P_{\mathcal{W}}(x) := \arg\min_{y \in \mathcal{W}} D_{\psi}(y, x)$.
\end{definition}
If $\mathcal{W}$ is convex and closed then the forward projection exists and is unique. Existence and uniqueness follow from continuity, boundedness of sublevel sets (Exercise 1 in \cite{fawzinotes}), and strict convexity of $D_{\psi}$ in its first argument. The following is a known generalization of the standard $\ell_2$ Pythagorean inequality to Bregman divergences.

\begin{fact}[Generalized Pythagorean Inequality \cite{dhillonnotes}] \label{thm:bg_pyth_main}
    Let $\mathcal{W} \subset U_{\psi}$ be a closed, convex set. Then for all $z \in U_\psi$ and $x \in \mathcal{W}$
    $$D_{\psi}(x, z) \geq D_{\psi}(x, P_{\mathcal{W}}(z)) + D_{\psi}(P_{\mathcal{W}}(z), z)$$
\end{fact}

\subsubsection{Expectations of Bregman Divergences}
\label{sec:exp_bregman}

Suppose we have a random variable $X \sim P_X$ with finite support $\mathcal{X}$. Functions $\mathcal{X} \to \sR^n$ form an $n|\mathcal{X}|$ dimensional vector space that we give the $L^2$ norm $\sqrt{\E \left[ \|f(X) - g(X)\|_2^2 \right]}$. From strictly convex, $C^1$, $\psi: \sR^n \to \eRp$, we get a convex functional $\Psi$ defined $\Psi[f] := \E[\psi(f(X))]$. Computing the dual map, Legendre dual, and Bregman divergence of $\Psi$, we get $f^* = \nabla \psi \circ f$, $\Psi^*[f^*] = \E \psi^*(f^*(X))$, and $D_\Psi(f,g) = \E D_\psi(f(X), g(X))$. Thus, the previous results about Bregman divergences also apply to \textit{expectations} of Bregman divergences when $|\mathcal{X}| < \infty$. See Appendix \Cref{sec:beyond-finite} for a discussion when $\mathcal{X}$ is not finite.


==> related-work.tex <==
\section{Related Work} \label{sec:related-work}

Our work is complementary to a growing line of works, each of which seeks to theoretically explain the phenomenon of weak-to-strong generalization via a different lens. The work of \citet{lang2024theoreticalanalysisweaktostronggeneralization} posits that the two crucial properties governing weak-to-strong generalization are \textit{coverage expansion} and \textit{pseudolabel correction}.
The work of \citet{somerstep2024statisticalframeworkweaktostronggeneralization} formalizes weak-to-strong generalization as the problem of transferring a ``latent concept'' from the weak model to the strong model. \citet{wu2024provable} show how finetuning a linear model on Gaussian features in the overparameterized regime provably exhibits weak-to-strong generalization. \citet{shin2024weak} take a data-centric approach, and propose that data points that contain an overlap of \textit{easy} as well as \textit{hard} patterns most effectively elicit generalization. \citet{ildiz2024high} recently provide a high-dimensional analysis of knowledge distillation from surrogate models. Our work adopts the geometric viewpoint of \citet{charikar2024quantifyinggainweaktostronggeneralization}, which interprets the finetuning of the strong model with weak labels as a \textit{projection} of the weak model onto the strong model class (where the projection corresponds to minimizing a loss function), conveniently allowing, for example, to incorporate convexity assumptions.

The main takeaway from our work about the gain in weak-to-strong generalization being characterized by the disagreement between the student and teacher model (an observation originally made empirically by \citet{burns2023weaktostronggeneralizationelicitingstrong}) aligns well with the general flavor of results in co-training \citep{blum1998combining} and disagreement-based generalization bounds \citep{dasgupta2001pac, wang2017theoretical, yu2019does}. Particularly relevant also is the vast literature on knowledge distillation (e.g., \citet{hinton2015distilling, nagarajan2023student}) and self-distillation (e.g., \citet{wei2020theoretical, mobahi2020self, pareek2024understanding}). It is worth mentioning that the work of \citet{lang2024theoreticalanalysisweaktostronggeneralization} draws insights from both \citet{blum1998combining} and \citet{wei2020theoretical}.




